Exploring the Potential of Multimodal LLM with Knowledge-Intensive Multimodal ASR

Recent advancements in multimodal large language models (MLLMs) have made significant progress in integrating information across various modalities, yet real-world applications in educational and scientific domains remain challenging. This paper introduces the Multimodal Scientific ASR (MS-ASR) task, which focuses on transcribing scientific conference videos by leveraging visual information from slides to enhance the accuracy of technical terminologies. Realized that traditional metrics like WER fall short in assessing performance accurately, prompting the proposal of severity-aware WER (SWER) that considers the content type and severity of ASR errors. We propose the Scientific Vision Augmented ASR (SciVASR) framework as a baseline method, enabling MLLMs to improve transcript quality through post-editing. Evaluations of state-of-the-art MLLMs, including GPT-4o, show a 45% improvement over speech-only baselines, highlighting the importance of multimodal information integration.

==> sections/0_abstract-old.tex <==
\begin{abstract}
% State-of-the-art Automatic Speech Recognition (ASR) models like Whisper have been successfully applied in a variety of scenarios, including the transcription of movie subtitles and daily phone conversations.
% However, content-rich scenarios, such as transcribing conference presentations, remain challenging for these state-of-the-art models. They may lack the necessary knowledge included in the presentation, especially when it involves new concepts or information unlikely to be found in the ASR model's training corpus.
% In this paper, we propose a flexible and transparent framework that uses LLM of different modalities to collaboratively process the content of vision, speech, and text, and eliminates potential information gaps through complementary information between modalities, thereby improving the quality of ASR transcripts.
% Meanwhile, we propose an explainable evaluation protocol to clarify the evaluation process. This protocol breaks down ASR errors into multiple dimensions, making them more interpretable than the WER.
% In our experiment, we demonstrate that our proposed framework effectively reduces critical ASR errors from 67\% to 13\%, particularly on terminologies and named entities.
% Automatic Speech Recognition (ASR) systems have made significant strides in recent years, yet they continue to struggle with content-rich scenarios such as conference presentation. 
% % You mean knowledge-rich scenarios?
% Integrating visual modalities offers a promising solution to these issues, but existing end-to-end models often lack interpretability. This paper presents the Interpretable Vision-Assisted ASR framework (InterVASR) based on multimodal large language models (LLMs) which not only enhances recognition accuracy but also ensures interpretability. 
% Additionally, to solve the inconsistency between WER and user preference on transcribed text, we propose an evaluation protocol that systematically assesses ASR from the severity of errors on user experience, providing a clear and quantifiable measure of the performance. 
% Human preference is a subjective term, maybe replace it with human evaluation

% Yuxia modification:
% Automatic Speech Recognition (ASR) systems have made significant strides in recent years, yet knowledge-rich domains remain challenging such as academic conference presentations. 
% We present a vision-augmented ASR framework (AcaVASR) to alleviate this problem by fully leveraging signals embedded in videos and knowledge stored in multimodal large language models (LLMs).
% It enhances recognition accuracy and interpretability, and also exhibits superior extensibility compared to end-to-end models in terms of efficiently adapting to unseen domains.
% In experiments, we observed the discrepancy between the evaluation metric WER and human assessments. To mitigate this gap, we propose an automatic evaluation approach, which assesses the quality of transcribed text from multiple perspectives including the mismatched content type, error severity and its semantic impact on understanding the whole speech. Both qualitative and quantitative measurements demonstrate high correlation with human judgment.


Automatic Speech Recognition (ASR) systems often struggle to accurately transcribe academic conference presentations 
% \textcolor{blue}{(Ehsan: same comment as title)} 
% TBD
due to complex jargon and diverse speaker attributes.
We introduce a vision-augmented ASR framework (AcaVASR) to alleviate this problem by fully leveraging information 
% \textcolor{blue}{(Ehsan: why the emphasis is on embedded signals here, it gives the impression of a work that looks at representations which is not the case here)}
embedded in vision modality and knowledge stored in multimodal large language models.
% \reza{multimodal large language models (LLMs)}\nreza{large multimodal models (LMMs)}
We empirically demonstrate that AcaVASR improves both recognition accuracy and interpretability. %
% \textcolor{blue}{(Ehsan: I am not sure if we can play the interpretability card, are we making ASR more interpretable? Or it is just that we require natural language communications between LLMs in the pipeline?)}. 
% MH: compared to end-to-end models, we can interpret what knowledge is used to correct the original ASR from intermediate scene-level and presentation-level summary. 
% , demonstrating enhanced extensibility over end-to-end models by efficiently adapting to new, unseen domains.
%In experiments, 
Additionally, we observe a discrepancy between the commonly used ASR evaluation metric WER, and human assessments. 
%was observed.
To mitigate this gap, we propose a more nuanced severity-aware evaluation protocol which assesses the quality of transcribed text from multiple perspectives including the content type and severity of the ASR errors, emphasizing their semantic impact on the overall understanding of the speech. 
% Both qualitative and quantitative measurements demonstrate high correlation with human judgment.
Our results demonstrate that AcaVASR provides a promising solution for content-heavy ASR applications. The evaluation protocol offers a more nuanced understanding of ASR performance, which is more aligned with human preferences.

% \textcolor{blue}{(Ehsan: Need a better finishing sentence as this repeats everything already stated above. Maybe: This, to the best of our knowledge, is the first attempt in utilising foundation models across speech, text, and vision modalities to improve ASR accuracy.)}
% MH: I'm not sure whether we are the first.


% Automatic Speech Recognition (ASR) systems often struggle to accurately transcribe academic conference presentations due to complex jargon and diverse speaker attributes. We introduce a vision-augmented ASR framework (AcaVASR) to alleviate this problem by fully leveraging contexts embedded in vision modality and knowledge stored in multimodal large language models. We empirically demonstrate that AcaVASR improves both recognition accuracy and interpretability. Additionally, we observe a discrepancy between the commonly used ASR evaluation metric WER, and human assessments. To mitigate this gap, we propose a more nuanced severity-aware evaluation protocol which assesses the quality of transcribed text from multiple perspectives including the content type and severity of the ASR errors, emphasizing their semantic impact on the overall understanding of the speech. Our results demonstrate that AcaVASR provides a promising solution for content-heavy ASR applications. The evaluation protocol offers a more nuanced understanding of ASR performance, which is more aligned with human preferences.
\end{abstract}




==> sections/1_intro-old.tex <==
\section{Introduction}
% Automatic Speech Recognition (ASR) models transcribe spoken language into text using audio input. Despite significant advancements, current state-of-the-art ASR systems still face significant challenges in knowledge-rich domains such as academic conference presentations. In these scenarios, ASR systems often lack sufficient domain knowledge, leading to the misrecognition of technical terms and named entities as incorrect homophones. While some errors can be mitigated by fine-tuning the model on domain-specific data, this approach is inherently limited. Domain knowledge has been evolving fast, particularly for exploratory scientific research. The speech of fine-tuning models to memorize new knowledge cannot catch up with the speed of knowledge changes. Additionally, the diversity in speakers’ accents, English proficiency, and fluency in conference recordings further complicates accurate recognition.

Automatic Speech Recognition (ASR) systems have significantly advanced, yet they continue to encounter substantial challenges in knowledge-rich domains like academic conference presentations. Traditional ASR systems often struggle to accurately recognize technical terminology and named entities, misinterpreting them as homophones due to a lack of specialized domain knowledge. 
% frequently mistaking them for homophones due to insufficient domain knowledge. 
While fine-tuning ASR models with domain-specific data can mitigate this issue, it is always hard to keep pace with the rapid evolution of technical domain knowledge.
%, particularly in fields characterized by exploratory scientific research. 
Moreover, the variability in speaker accents, proficiency in English, and speech fluency in conference speech recordings exacerbate the complexity of transcription.
%
\begin{figure}
    \centering
    \resizebox{0.9\columnwidth}{!}{%
        \includegraphics{figures/overall_example.pdf}
    }
    \caption{Why visual contexts are important to ASR.}
    \label{fig:visual_context_importance}
    \vspace{-1em}
\end{figure}
%
%
 %
For instance, as the example in Figure \ref{fig:visual_context_importance} demonstrates, the ASR system operating on the audio input recognizes \textit{BERT} and \textit{RoBERTa} as \textit{birds} and \textit{robots} because it does not know the names of two well-known language models in NLP. However, presentation slides often contain the concepts being discussed, providing contextual support that can enhance ASR accuracy. 
% \textcolor{blue}{(Ehsan: is this a hypothetical exmaple? If it is, why not put a real example in the figure and cite what ASR system procudes the error?)} 
% MH: This is a real example, but the slide content is too dense, which is not clear to show what we want to present.

% \textcolor{blue}{(Ehsan: the logic here seems a bit broken as the emphasis is placed on the \emph{contextual support} rather than the \emph{explicit visual cue} in the slides spelling BERT and RoBERTa. Context is important, but you also need to connect this to the explicit information that is present on each slide.)}
% MH: the demonstration example should be intuitive for reader to understand the major idea of our method, instead of comprehensively demonstrating all advantages or features of the method in my view, and the context is not easy to be plotted in this figure.

% Therefore, recent studies have increasingly explored the integration of supplementary visual information to improve ASR performance. \citet{oneata2022improving,ghorbani2020listen,seo2023avformer,gabeur2022avatar,caglayan2019multimodal} developed end-to-end models processing audio and visual inputs simultaneously.
% are most of them end-to-end models, can we say:

Recent studies have increasingly explored the integration of supplementary visual information to improve ASR performance, particularly by training end-to-end models which capture audio and visual signals simultaneously~\citep{oneata2022improving,ghorbani2020listen,seo2023avformer,gabeur2022avatar,caglayan2019multimodal}.
However, these models suffer from three primary limitations: (\emph{i}) unable to process long videos (i.e., maximum limit of 30 seconds),
% Add citation about 30 seconds VASR studies
while even a short paper presentation is at least 10 minutes. Though slicing a long video into smaller chunks could enable the process, it will lose the contextual information from earlier chunks, sacrificing accuracy of context-dependent segments.
% 
% \textcolor{blue}{(Ehsan: why could they not just slice video into smaller chunks? what would be sacrificed by doing this? I think we also have the same limitation as we are relying on transformer encoders. Maybe you need to capitalize the significance of \emph{missing contextual information} in previous systems instead, assuming they did not explicitly capture or inject context outside of the 30 seconds window while you are practically incorporating the whole thing via text LLM/summary.)}
% 
(\emph{ii}) skilled at capturing and interpreting a series of movements of an object in videos but not proficient in handling information-intensive speech due to the biased distribution of available training data, and (\emph{iii}) high computational expense to adapt to new domains and learn new knowledge, which makes the adaption of end-to-end models to conference presentation ASR challenging.
% \textcolor{blue}{(Ehsan: again not too sure you should be focusing on this explicit task in your problem statement ... this could be kept at a high more fundamental level, till you get to the experimental finding paragraph of the introduction)} 

To fill the gap of integrating visual information into ASR systems that can be effectively adapted to content-rich scenarios, e.g., academic conference presentations, we propose AcaVASR, a vision-augmented zero-shot ASR framework. 
On one hand, it leverages textual cues extracted from visual data; on the other hand, it makes a full use of parametric knowledge stored in textual large language models (LLMs) to enhance transcripts generated by a baseline ASR model, such as \model{Whisper}. 
Most importantly, AcaVASR integrates contexts of the whole speech. It is crucial to overcome the limits of prior work -- transcribing technical terms that are not explicitly presented in the current video slice but appeared in earlier chunks. 
AcaVASR effectively enables transcriptions of long recordings by low computational overhead efficiently, bringing 45\% improvements in the transcript quality.
% \textcolor{blue}{(Ehsan: what about highlighting the incorporation of long context beyond previous works limit? This seems quite important as some of the technical terms uttered by the speaker may have been introduced in earlier parts of the recording and not appearing on the  explicit slide at this given time step.)}
% \reza{Most importantly, AcaVASR enables effective transcriptions of long recordings by low computational overhead efficiently.
% }\nreza{need to mention how (the appraoch/technique)}
%
% \textcolor{blue}{(Ehsan: have 1-2 sentences at the end of this paragraph and highlight what empirical improvements (\%) is achieved by your method.)}


In experiments, we further observed that conventional ASR evaluation metrics like Word Error Rate (WER) is not aligned with human preferences in particular for knowledge-intensive ASR settings.
% \textcolor{blue}{(Ehsan: maybe safer to contextualize this statement: ... is not aligned with human evaluation in particular for knowledge-intensive ASR settings.)})
WER treats all errors equally, failing to distinguish between critical and minor mistakes. For instance, the misrecognition of technical terms that significantly impact the correct understanding of the sentence is more severe than missing an \textit{ah} or recognizing \textit{the} as \textit{this}.
% ---------------------
This drawback is particularly pronounced in academic settings.
% \textcolor{blue}{(Ehsan: suggest dropping this sentence)}).
% MH: Why?
% ---------------------
Therefore, we introduce a more nuanced 
% \textcolor{blue}{(Ehsan: changing \emph{new} with \emph{more nuanced})})  
evaluation framework that assesses ASR predictions from the type and severity of errors, emphasizing the impact on semantic comprehension. Results show that evaluations by this approach better align with human preferences.
% \trang{user preferences}\ntrang{user preferences or human evaluation?}. 
Meanwhile, the comprehensive analysis allows the tracking of errors, demonstrating apparent improvements brought by visual inputs quantitatively.
% \textcolor{blue}{(Ehsan: meant to say quantitatively?)})

The contributions of this paper are threefold.
\begin{itemize}
% \begin{compactitem}
    \item We introduce a zero-shot framework AcaVASR that integrates text and vision modalities to enhance ASR accuracy in knowledge-intensive settings. %, without domain-specific tuning.
    \item We propose a more fine-grained ASR evaluation framework. It can systematically assess transcription accuracy across multiple dimensions, closely reflecting human preferences.
    \item Experiments show the effectiveness of both AcaVASR and evaluation framework, code is available at \textit{URL withheld}.
% \end{compactitem}
\end{itemize}




    % \textcolor{blue}{(Ehsan: suggest replacing \emph{a cascade pipeline} with \emph{a zero-shot framework})}
    
    % \textcolor{blue}{(Ehsan: same comment as above ... this is too narrow)}
   
    
    % \textcolor{blue}{(Ehsan: suggest replacing \emph{innovative} with \emph{more fine-grained} )}
    
    % \trang{user preferences}\ntrang{user preferences or human evaluation?}
    


% \textcolor{blue}{(Ehsan: Need a finishing statement, highlighting that while your empirical setting is focused on academic conference presentation, there is a much bigger potential for impact in similar content-heavy deployment environments such as X, Y, Z.)}





\begin{comment}

% fall short in handling extended recordings typical of conference presentations, primarily due to their limitations in processing long videos and a focus on motion rather than content-rich visuals. Therefore, approaches that focus on content-rich long videos are still under-explored.

% End-to-end model limitations
% Incapable of processing long videos
% Motion-rich video rather than content/knowledge-rich videos
% High cost to perform domain adaptation
% Data scarcity in narrow domains

% \citet{oneata2022improving,ghorbani2020listen,seo2023avformer,gabeur2022avatar,caglayan2019multimodal} have utilized visual modalities to assist ASR, primarily by developing end-to-end models that could process audio, images, or video frames in parallel to generate transcripts.
% However, these end-to-end models are not suitable for scenarios such as conference presentations because of two critical drawbacks: (\emph{i}) Most end-to-end models are only able to process short video clips less than 30 seconds, but a presentation recording may last more than 10 minutes which poses a great challenge to these models. (\emph{ii}) Previous studies focus more on motion-rich videos instead of content-rich videos, this is to say, we need to tune the model on domain-specific datasets if we want to apply these models to content-rich videos. However, such datasets are very scarce, making domain adaptation difficult.
% Therefore, approaches that focus on content-rich long videos are still under-explored.


% From the perspective of evaluation, current ASR metrics such as Word Error Rate (WER) are also not suitable for the evaluation of knowledge-rich domains, because it treat all recognition errors equally, which sometimes fails to reflect the true performance of the model. For instance, misrecognizing ten technical terms has a vastly different impact on user understanding compared to misrecognizing ten simple words like “the” or “a.”


Additionally, traditional ASR evaluation metrics like Word Error Rate (WER) do not adequately reflect the nuances of knowledge-rich domains. WER treats all errors equally, failing to distinguish between the misrecognition of complex technical terms and simpler, less impactful words.

Given these challenges, our paper seeks to address two main research questions:
\begin{itemize}
    \item How can the vision modality be effectively integrated into ASR tasks for academic conference scenarios, which are rich in specialized knowledge?
    \item What methods can be developed to evaluate ASR systems that reflect the actual impact of transcription errors on user experience, especially distinguishing between critical and minor errors?
\end{itemize}

We propose AcaVASR, a vision-augmented ASR framework that leverages vision and text large language models (LLMs) to enhance initial transcripts generated by the \model{Whisper} model. This system refines transcripts using textual cues extracted from visual data, enabling efficient processing of extended recordings without the computational overhead of traditional methods.

Our framework operates in a zero-shot fashion, utilizing the pre-existing knowledge encapsulated within large language models (LLMs), thus eliminating the need for additional training. It is specifically designed to handle the unique challenges of long-duration academic presentations, efficiently condensing necessary information into manageable text segments.

Furthermore, we introduce a user-centric evaluation framework that assesses ASR predictions by the type and severity of errors, focusing on those that significantly affect comprehension. This framework not only tracks improvements brought by visual inputs but also aligns evaluation metrics more closely with user preferences.

The contributions of this paper are twofold:
\begin{itemize}
    \item Introduction of AcaVASR, a cascade framework that seamlessly integrates text and vision-LLMs to enhance ASR accuracy in academic settings without the need for domain-specific tuning.
    \item Development of an innovative ASR quality evaluation protocol that systematically assesses transcription accuracy across multiple dimensions, providing a more accurate reflection of user experience.
\end{itemize}

\end{comment}





==> sections/3-method-old.tex <==
\section{AcaVASR}
\label{sec:method}

\begin{figure*}[t]
    \centering
    \resizebox{0.8\textwidth}{!}{%
        \includegraphics{figures/vmt_architecture.pdf}
    }
    \caption{\textbf{The architecture of AcaVASR.} \textbf{Baseline ASR} model transcribes a presentation recording into a transcript. \textbf{Video segmenter} splits video frames into a sequence of scenes with each presenting a slide. \textbf{Slide analyzer} applies multimodal LLMs to extract key information from scene images into visual contexts represented by text. \textbf{Post-editor} instruct a text-LLM to leverage visual contexts to refine the ASR transcript.} 
    % \trang{TV: what is the scene-level and presentation-level summary in the figure?}
    % \textcolor{blue}{(Ehsan: Mention in the caption the example slide is taken from XXX dataset with a citation. Also what is MLLMs? It was never introduced in the text.)} 
    \label{fig:architecture}
\end{figure*}


In this section, we first introduce the task formulation that our framework aims to solve, followed by the detailed description of the architecture.

\subsection{Task Formulation}

In this work, we focus on the ASR task for conference presentation recording videos. 
Instead of following the conventional formulation to recognize sentence-level utterances based on well-split speech segments, we treat each video as a whole and generate a presentation-level transcript for the entire video.
Such task formulation aims to evaluate the accuracy of the ASR system on long videos and also aligns better with the real-world application setup which does not provide pre-segmented utterances.

% We utilize the ACL 60/60 dataset~\citep{elizabeth2023acl6060}, which comprises video recordings of accepted papers at ACL 2022. 
% \trang{TV: This is more of dataset introduction than task formulation. A task formulation should not bind to a specific dataset}.

% The reason is that the segmentation timestamps often have finer granularity, which does not align well with the slide content presented in the video.


% Although the dataset provides well-segmented speech utterances, we chose not to use these segments. The reason is that the segmentation timestamps often have finer granularity, which does not align well with the slide content presented in the video. Therefore, unlike conventional approaches that infer sentence-level utterances, we treat each video as a single sample and aim to generate a document-level transcript for the entire video.


\subsection{Architecture}
% The architecture of AcaVASR consists of four components, corresponding to four subtasks and organized in a pipeline manner.
AcaVASR consists of four components, corresponding to four sub-tasks, and is organized in a pipeline manner, as shown in Figure \ref{fig:architecture}.
% \reza{Figure~\ref{fig:llm_evaluation_case}.}\nreza{Figure 2?}

\subsubsection{Baseline ASR}
Firstly, a state-of-the-art ASR model, such as \whisperbase~\citep{radford2023whisper}, is employed to transcribe the video's speech into text along with corresponding timestamps. 
% Despite high-quality transcripts by Whisper, there are still numerous errors. They will be addressed in the subsequent steps.

\subsubsection{Video Segmenter}

In contrast to motion-rich videos, where each frame contributes to the depiction of a continuous movement, presentation recordings are typically composed of static scenes with slides presented by the speaker. 
To reduce the complexity and computational cost of the pipeline, we segment the video into a sequence of scenes, with one slide representing the visual context of each scene.
% To reduce the complexity and computational cost of the pipeline, we segment the video into a sequence of scenes featuring by slide content, and sample a single frame to represent each scene.

% \textcolor{blue}{(Ehsan: this last bit is unclear ... do we have several scenes featuring the same slide? if so, the next statement needs to be adjusted to \emph{and sample a single frame to represent the entire sequence of scenes containing the same slide})}
% MH: Not necessarily, the scene and slides are not always bi-mapped.

Specifically, we first apply the Kernel Temporal Segmentation (KTS) algorithm~\citep{DBLP:conf/eccv/PotapovDHS14,DBLP:conf/iccvw/AfhamSPZSL23} on the video frame features extracted by a pretrained image encoder, e.g., \model{CLIP}~\citep{radford2021clip}. KTS derives the optimal segmentation policy by identifying the boundaries (change points) of each scene from the video frames. The output of KTS is a sequence of consecutive time spans in seconds, with each span indicating the start and end times of a scene.

We find that the predicted scene boundaries align well 
% \textcolor{blue}{(Ehsan: need some quantification - maybe as a footnote you can report a metric indicating exactly how much this aligns on what dataset)}
with the moment when the speaker moves to the next slide. Therefore, for each scene, we sample a frame image at 90\% of the time span before the speaker moves to the next slide. This aims to ensure that the sampled frame contains the complete textual content of the slide even if there were animations.
Processing only 10-30 scene images instead of all video frames significantly reduces computational demands without losing key information.
% \textcolor{blue}{(Ehsan: does this not introduce segmentation latency? where do we discuss this?)}
The scene time spans also guide the segmentation of transcripts corresponding to each slide.
Ultimately, we obtain a sequence of scenes \(\mathcal{S} = [S_1, ..., S_N]\), where \(N\) is the number of scenes. Each scene is represented by a tuple \(S_i = (\mathcal{I}_{i}, \mathcal{T}_{i})\) with the slide image \(\mathcal{I}_{i}\) and the corresponding transcripts \(\mathcal{T}_{i}\), where \(i\) is the scene index.
% \reza{ % within the time span
% }\nreza{For each scene $S_i=(I_i,T_i)$, what if during the scene $S_i$ there as an animation in the slide? (do you keep all of those images as an image 'set' and assign it to $I_i$?) }
%\ntrang{I believe that only a single image sampled at 90\% timespan, i.e. when all animations are completed. However, there would be a scenario where the animation removes information from the slide.}

\subsubsection{Slide Analyzer}

The slide analyzer is a critical component in this framework. It extracts visual information from the segmented scene images and transforms visual context into natural language. These textual representations of scenes act as auxiliary references for transcript refinement, and are also used to interpret how visual context affects ASR transcripts. 


% This component is critical in our framework as it transforms visual context into textual representation. The intermediate results produced by this component serve as textual evidence to interpret how visual context affects ASR transcripts. The intuition behind this stage is to use a vision-LLM to perform visual information extraction from the segmented scene images.

\paragraph{Visual Context Extraction}

A text-LLM and a vision-LLM collaborate to extract the required visual contexts from the slide images. 
The necessity of using LLMs in both modalities instead of only a vision-LLM lies in the fact that many state-of-the-art vision-LLMs cannot handle complex reasoning tasks, particularly when dealing with false-premise or unanswerable questions.
For example, when the vision-LLM is asked to provide the affiliation of the author, it sometimes hallucinates an incorrect institution as it is not able to deduce the relation between the author's name and the institution's name presented on the slide as affiliation. However, if asking it to list bullet points, it can extract the correct institution name.
% \textcolor{blue}{(Ehsan: is there any study that shows visionLLMs are more prune to hallucination than textLLMs?)} 
% ----------------------
% TODO: cite paper about MLLMs hallucination
% ----------------------
% YX: why we have unanserable and misinformation questions?
In contrast, text-LLMs are superior in reasoning and are more robust in these situations. Combining both types of LLMs offers a positive complementary effect.

% \textcolor{blue}{as they are solely trained on text data, although still have potential to hallucinate content}.
%misinformation.

%ensures the quality of extracted contexts.
 

% In this stage, a text-LLM and a vision-LLM collaborate to extract the required visual contexts from the slide images. The necessity of using LLMs in both modalities, rather than relying solely on a vision-LLM, lies in ensuring the quality of extracted contexts. Many state-of-the-art vision-LLMs can handle simple document understanding tasks but often fail in complex reasoning tasks, particularly when dealing with questions containing misinformation or unanswerable questions. In contrast, text-LLMs excel in reasoning and are more robust to misinformation, making them essential for this stage.

% Specifically, we employ three strategies to instruct the vision-LLM to extract information from the slide images:
% Present only one strategy 


% \begin{itemize}
%     \item \textbf{Simple OCR} The vision-LLM is prompted to perform OCR on the given image.
%     \item \textbf{General Question Answering} Eight predefined questions covering aspects such as layout, title, bullet points, figures, and tables in the slide (detailed in Appendix A) are used to prompt the vision-LLM to extract relevant information into specific answers.
%     \item \textbf{Ad-hoc Question Answering} The text-LLM first identifies possible errors in the transcript of the current page and generates ad-hoc questions to clarify confusing parts. The vision-LLM then answers these questions based on the slide image.
% \end{itemize}

Specifically, we predefine eight questions covering aspects such as layout, title, bullet points, figures, and tables in the slide are used to prompt the vision-LLM to extract relevant information by specific answers (see questions in Table \ref{tab:predefined_questions} of Appendix \ref{sec:app-implement-detail}).
These answers are often granular, duplicative, excessively lengthy, and even contain misinformation (see an example in Appendix~\ref{??}).
% \textcolor{blue}{(which appendix?)}
Therefore, we regard them as raw contexts, and further leverage a text-LLM to cross-validate, correct inaccuracies caused by the vision-LLM hallucinations, and summarize the lengthy raw contexts into a concise summary, referred to as the scene-level context $\mathcal{C}_{i}$.
This summary is added to the scene tuple: $S_i = (\mathcal{I}_{i}, \mathcal{T}_{i}, \mathcal{C}_{i})$. % repeated S, change one of them.


% The outputs from the vision-LLM are considered raw contexts. These raw contexts are often granular, may contain misinformation, and can be duplicative, resulting in excessive length. Therefore, we need to condense them into appropriate granularity.
% The text-LLM can cross-validate cues within the raw contexts, correcting misinformation caused by the vision-LLM's hallucinations. Here we use the text-LLM to summarize the raw contexts for each scene into a natural language summary, referred to as the scene-level context, denoted as $\mathcal{S}_{i}$. This summary is then added to the scene information tuple: $S_i = (\mathcal{I}_{i}, \mathcal{T}_{i}, \mathcal{S}_{i})$.

\paragraph{Visual Context Condensement}

For some scenes, information on the current slide may not be helpful in correcting errors in the corresponding transcripts since the relevant cues appear in earlier slides.
That is, a longer context window is needed. Therefore, we use the text-LLM to further condense scene-level summaries into an overall presentation-level summary to share temporal contexts across scenes. This is achieved by prompting the text-LLM to generate a comprehensive summary based on the concatenated scene-level summaries, denoted as $\mathcal{P}$.
Both scene-level and presentation-level summaries will be passed to the next step: post-editing.


% Thus, the visual information extraction process is complete, and the extracted information will be used for the post-editing of ASR transcripts.

\subsubsection{Post-editor}
In the post-editing stage, we instruct the text-LLM to utilize the extracted visual context $\mathcal{C}_i$ and $\mathcal{P}$ to correct errors in the ASR transcript $\mathcal{T}_i$ (See prompts in Figure \ref{fig:post_editing_prompt} of Appendix \ref{sec:app-implement-detail}). % see prompts in xxx
% This also operates at the scene level with the input $(\mathcal{T}_i, \mathcal{S}_i, \mathcal{P})$. 
The output of the post-editor for each scene is denoted as $\hat{\mathcal{T}}_{i}$. $\sum_{i=1}^{N} \hat{\mathcal{T}}_{i}$ constitutes the final output. 

% We prompt the text-LLM to return the post-edited transcript given the input context formatted appropriately.
% \begin{itemize}
%     \item \textbf{Direct PE} In this strategy, we prompt the text-LLM to return the post-edited transcript given the input context formatted appropriately.
%     \item \textbf{Chain-of-Thought PE} Instead of merely requesting the post-edited transcript, we prompt the text-LLM to first provide comprehensive correction records for each identified error, including the reason for the correction, followed by the post-edited transcript.
% \end{itemize}


==> sections/annotation.tex <==
% Annotation summary:
% A debate between keeping genuine or grammarly correct. Should we strictly translate based on the user’s speech, or should we make it correctly in grammar.
% Optimize the algorithm to label <>, {}, []
% Context-dependent: for example:
% [auto completion] [to guess] -> [autocompletion,] [the gas], instead of like the original split as [auto completion to guess], <>
% Original: by {training} a [single] online parser -> by {} a [truney-as-single] online parser
% Revision: by <> [training a single] online parser -> by <a> [truney-as-single] online parser
% 110: line 113, 429
% 117, line 182 (captains of)
% 111, line 37, 450, 588, 671, 871 … too many, rerun the 111 please.
% 111 speech line 450: Seemingly because there’s \ in the gold text that all {} [] <> are labeled ahead of its correct position. Some errors made by mismatch algorithm are fixed the the LLM,
% Context-independent: Normalize words like 45 to forty five, under explored to underexplored, we’ re to we are, two-step -> two step. For such context-independent normalization can be done after matching, filter these erroneous candidates out.
% Miss mismatch with small edit distance (in 117):
% Revision: [of] -> [or]
% Revision: [captains of] -> [captain's or]
% Some errors made by mismatch algorithm are fixed the the LLM,
% Check the relationship between mismatch_content_type with severity, models may always considers grammatical words as “OK”
% Consistency of the evaluation, for example, same words, same functionality, labeling difference severity between paragraphs.
% Maybe specify more clearly for mismatch_content_type.
% The word itself or its function in this context: some are general words, such as find or fine, but they are the name of a function they defined, how could we label them, as general words or terminology or entity?
% Word content type or error type: sometimes the content is a general word, but the error it makes is a grammar mistake, like propose a -> proposed the, or happening to happen, and self-pointing -> self pointing. I think it is grammar error and minor/ok, instead of general words,
% We may need to adjust the evaluation prompts later afterwards accordingly.
% From the annotation accuracy perspective, non-expert annotator in NLP may produce results that are more aligned with the annotation guideline we give LLM in prompt, additionally, it might be easier for layman to distinguish terminology from general words than experts, because experts have got used to the terminology, they may regards them as general words that frequently occur in their daily life.

==> storyline.tex <==
% % May 08 2024
% % Discussed storyline
% Our case study show that even the state-of-the-art speech-to-text model Whisper makes significant number of errors such as (like the top 5 error types, type 1 refer, 2, 3 ..), especially non-native speakers with accent and low fluency. 
% Error type 1 and 2 are mainly attributed to ambiguous reference shown in the video image, and the type 3 is due to poor identification of new terminology. 
% To alleviate these issues, we propose to incorporate video information to help ... and leverage knowledge stored in LLMs to fix the terminology.

% Our experiments show ..., but existing evaluation metrics can only show a numerical score indicating that the quality of the outputs might be improved or degraded by editing distance, it can not demonstrate what errors the system make, and how many are critical, how many are less important and can be neglected, whether the proposed methods can potentially solve the problems.
% Furthermore, what errors are solved, what are not, what new errors are introduced by the enhancement methods.
% To this end, we propose a new evaluation framework. It can offer comprehensive analysis to compare the gold transcripts and the predicted one. 

% Experiments show that evaluation based on small models can achieve similar accuracy as prompt-based LLM evaluator when tuning it with xx k examples.


% To sum, there are three major contributions:
% (1) we propose a method to improve the output quality of speech-to-text translation by incorporating information of images in the video, and leveraging the LLM parametric knowledge. The enhanced outputs are more aligned with speech with less errors, especially in the terminology and ...
% (2) we propose an automatic evaluation framework assessing the outputs of speech-to-text models comprehensively, from the perspective of the total number of errors, specific error type, rationale behind the error, and potential solutions for how to fix the error, for example, depending on the video information and knowledge in LLMs investigated in our paper.
% (3) we conduct comprehensive analysis in terms of what errors are fixed by our methods, what errors are remained, and what new errors are inducted by comparing triplets (gold transcripts, vanilla outputs, enhanced outputs). 
% The analysis show that ...
% We automated the analysis procedure and visualize it in a demonstration system.
% We believe both the evaluation and analysis framework will make speech-to-text evaluation more accurate, fine-grained, transparent, and intuitive, promoting the development of this domain.   





% \section{About Vision Part}
% There are two things correlated to vision in our framework.
% \begin{itemize}
%     \item Scene Segmentation
%     \item Scene Analysis
% \end{itemize}

% \subsection{Scene Segmentation}
% It is not that difficult to evaluate the accuracy of the segmentation method, we use human annotation to annotate the accurate page-turn timestamp, and compute a difference between the predicted scene time and ground-truth scene time.



% \subsection{Scene}
% For errors caused by the lack of specific knowledge in ASR model, external information coming from visual content can be helpful during the post-editing process. But we need to understand it works in what circumstances.

% For the current framework, the visual contents are extracted from a vision-LLM. There are two properties we should focus on:
% \begin{itemize}
%     \item The Completeness of the extracted content (Recall)
%     \item The Quality of the extracted content (Accuracy)
% \end{itemize}

% To evaluate the recall of vision-LLM, we can use GPT4-V and human annotation to create ground-truth labels for each slide.




% \section{About ASR Errors}
% A clear ASR error taxonomy should be the breakthrough for us to understand the evaluation result, as it gives us an insight to break down the performance of an ASR system from a confused overall score into some interpretable cues.
% Current ASR error classification/taxonomy is still quite trivial, they use \textbf{Insertion/Substitution/Omission} error to classify errors in ASR transcripts. However, this approach is just breaking down the computation of WER but not consider the semantics of words and the criticalness of errors. To have a clear understanding on ASR performance and how critical the errors made by ASR lead to misunderstanding, we propose the following ASR error taxonomy, to guide the annotation of human or LLM to perform ASR error classification. 

% \subsection{ASR Error Taxonomy}

% We have developed a clear and structured classification system to categorize the mismatches identified between ASR transcripts and their ground truth. This system includes the following categories:
% \begin{itemize}
%     \item \textbf{Terminology}: Specialized words or phrases used extensively within a specific field or industry.
%     \item \textbf{Key Words}: Words that carry the primary meaning essential for understanding the main themes or arguments of the text.
%     \item \textbf{Numerical Data}: Numbers, dates, quantities, or statistical data that provide specific, quantifiable details.
%     \item \textbf{Named Entities}: Proper nouns including names of people, places, and institutions that are critical for identifying specific details within the document.
%     \item \textbf{Function Words}: Words that primarily fulfill a grammatical role, such as prepositions, conjunctions, articles, and auxiliary verbs.
%     \item \textbf{Modal and Filler Words}: Words that express modality or are used as fillers, which do not significantly alter the meaning of the sentence but reflect the speaker’s tone or hesitation.
%     \item \textbf{Other}: A reserved category for mismatches that do not fit into the other defined categories, capturing unusual or rare usage that might be emerging or non-standard.

% \end{itemize}

% This classification is aimed at systematically analyzing mismatches in ASR transcripts to ensure each type of mismatch is accurately identified and categorized, thereby facilitating a detailed understanding of errors and supporting targeted improvements in ASR systems.

% \subsection{Semantic Impact Annotation Guidance}

% We defined a method to annotate and measure the severity of the impact of each mismatch on the speaker's intended meaning. This method involves:
% - Assessing each mismatch based on how much it changes the meaning of the text.
% - Grading the impact on a scale from 1 to 5, where 1 indicates no change in meaning and 5 indicates a complete change or misrepresentation of the intended information.

% This annotation approach allows for a quantitative assessment of the semantic impact of mismatches, providing insights into the precision and reliability of ASR systems in preserving the speaker's original intent. This will help in identifying critical errors that significantly affect the understanding of the transcript and prioritizing them for correction.

% These two key outcomes from our discussions provide a robust framework for deeper and clearer analysis of ASR system performance, enhancing both the evaluation and improvement of speech recognition technologies. This structured approach to analyzing and annotating mismatches will assist researchers, developers, and end-users in better understanding and managing the capabilities and limitations of ASR systems.




% \section{0514 Meeting Issues}
% \paragraph{Literature Review} Do a literature review on other multimodal ASR error correction papers, find the difference between ours and theirs, and illustrate why we cascade LLMs (content-heavy, knowledge intensive, long-form generation, etc.) instead of building an end-to-end model, what is the advantage of doing in this way.

% \paragraph{Refine the evaluation protocol} Reading the M2M paper, borrowing some ideas from explainable MT evaluation. Use binary classification instead of 1-5 scoring on the semantic impact evaluation, since it might be very subjective to obtain that score from human annotators or LLM. Design an experiment, justifying the taxonomy and semantic impact aligns with human annotation /user experience.


% \subsection{Related Work in Quality Estimation}
% There is not much work trying to propose an explainable evaluation protocol on ASR transcripts. However, for MT evaluation, many works are trying to do so. That means we can borrow some ideas from them.

% \paragraph{MQM}


% \paragraph{XComet} It covers both sentence- and lexical-level QE. For word-level QE, they predict a severity tag containing four levels [OK, MINOR, MAJOR, CRITICAL]. For sentence-level QE, they predict a score trained with the regression task on SRC, REF and SRC+REF. Meanwhile they also use the count of word-level tags to compute an MQM score as such:
% \begin{align}
%     e(S) &= c_{\text{MIN}} + 5 \times c_{\text{MAJ}} + 10 \times c_{\text{CRIT}}
%     \hat{y}_{\text{MQM}} = \frac{25 - e(S)}{25} if e(S) < 25 else 0
% \end{align}
% The final score is computed by a weight sum on $\hat{\textbf{y}} = [\hat{y}_{\text{SRC}}, \hat{y}_{\text{REF}}, \hat{y}_{\text{SRC+REF}}, \hat{y}_{\text{MQM}}]$:
% \begin{align}
%     \hat{y}_{\text{SL}} = \textbf{w}^{T}\hat{\textbf{y}}
% \end{align}
% The advantage of this evaluation approach is that it explicitly identifies the translation errors in the text and tags them with a severity label. However, it doesn't distinguish the content of the error, which is not helpful enough for researchers to conduct further analysis.



==> tables/pre-exp-perf.tex <==

\begin{table*}[]
\centering
\resizebox{0.9\textwidth}{!}
{%
\begin{tabular}{@{}c|cc|cc|cc|cc|cc|cc|cc@{}}
\toprule
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\textbf{\texttt{Whisper-base}}} & \multicolumn{2}{c|}{\textbf{\texttt{Whisper-large}}} & \multicolumn{2}{c|}{\textbf{Text-PE (Open)}} & \multicolumn{2}{c|}{\textbf{Text-PE (GPT-4o)}} & \multicolumn{2}{c|}{\textbf{Vision-PE (Open)}} & \multicolumn{2}{c|}{\textbf{Vision-PE (GPT-4o)}} & \multicolumn{2}{c}{\textbf{E2E-Vision-PE (GPT-4o)}} \\ \midrule
\textbf{VID} & \textbf{WER} & \textbf{TR} & \textbf{WER} & \textbf{TR} & \textbf{WER} & \textbf{TR} & \textbf{WER} & \textbf{TR} & \textbf{WER} & \textbf{TR} & \textbf{WER} & \textbf{TR} & \textbf{WER} & \textbf{TR} \\ \midrule
\textbf{110} & 14.41 & 86.06 & 14.76 & 91.02 & 15.11 & 87.88 & 13.18 & 93.94 & 15.58 & 92.12 & 11.89 & 95.76 & 13.01 & 95.76 \\
\textbf{117} & 11.16 & 89.11 & 15.47 & 90.86 & 13.00 & 88.71 & 9.70 & 91.13 & 16.47 & 89.52 & 9.43 & 93.95 & 10.40 & 94.76 \\
\textbf{268} & 18.58 & 85.92 & 24.38 & 88.88 & 19.61 & 90.29 & 17.01 & 92.72 & 19.94 & 93.69 & 16.79 & 97.57 & 18.96 & 97.57 \\
\textbf{367} & 17.99 & 76.44 & 16.78 & 80.34 & 15.95 & 81.33 & 14.57 & 84.89 & 16.10 & 86.22 & 13.77 & 85.78 & 14.93 & 86.67 \\
\textbf{590} & 14.44 & 95.73 & 19.63 & 93.61 & 15.35 & 96.58 & 13.45 & 96.58 & 14.77 & 96.58 & 13.37 & 97.44 & 17.00 & 92.31 \\ \midrule
\textbf{AVG} & 15.32 & 86.65 & 18.20 & 88.94 & 15.80 & 88.96 & 13.58 & 91.85 & 16.57 & 91.63 & 13.05 & 94.10 & 14.86 & 93.41 \\ \bottomrule
\end{tabular}%
}
\caption{This table presents results on the development set showing the result in WER and Term-Recall (TR) for each video, with average values presented in the last row.}
\label{tab:preliminary_exp_perf}
\end{table*}
